Improving Robust Generalization by Direct PAC-Bayesian Bound Minimization

Recent research in robust optimization has shown an overfitting-like phenomenon in which models trained against adversarial attacks exhibit higher robustness on the training set compared to the test set. Although previous work provided theoretical explanations for this phenomenon using a robust PAC-Bayesian bound over the adversarial test error, related algorithmic derivations are at best only loosely connected to this bound, which implies that there is still a gap between their empirical success and our understanding of adversarial robustness theory. To close this gap, in this paper we consider a different form of the robust PAC-Bayesian bound and directly minimize it with respect to the model posterior. The derivation of the optimal solution connects PAC-Bayesian learning to the geometry of the robust loss surface through a Trace of Hessian (TrH) regularizer that measures the surface flatness. In practice, we restrict the TrH regularizer to the top layer only, which results in an analytical solution to the bound whose computational cost does not depend on the network depth. Finally, we evaluate our TrH regularization approach over CIFAR-10/100 and ImageNet using Vision Transformers (ViT) and compare against baseline adversarial robustness algorithms. Experimental results show that TrH regularization leads to improved ViT robustness that either matches or surpasses previous state-of-the-art approaches while at the same time requires less memory and computational cost.

==> 08_Acknowledgement.tex <==
\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.


==> Tables/table_awpt.tex <==
\begin{table*}[!t]
\small
\centering

\begin{tabular}{lcccc|cccc}
\\
\toprule
\toprule
$\ell_\infty (\delta= 8/255)$  & \multicolumn{4}{c|}{ViT-L16}                            & \multicolumn{4}{c}{Hybrid-L16}       \\ 
\footnotesize{SE}$=\se{0.5}$\% &
  \multicolumn{2}{c}{CIFAR-10} &
  \multicolumn{2}{c|}{CIFAR-100} &
  \multicolumn{2}{c}{CIFAR-10} &
  \multicolumn{2}{c}{CIFAR-100} \\ 
Defense &
  \texttt{Clean}(\%) &
  \texttt{AA}(\%) &
  \texttt{Clean} (\%)&
  \multicolumn{1}{c|}{\texttt{AA}(\%)} &
  \texttt{Clean}(\%) &
  \texttt{AA}(\%) &
  \texttt{Clean} (\%)&
  \texttt{AA}(\%) \\ \midrule
AT(\AWP)     &88.5& \multicolumn{1}{c|}{\textbf{62.4}} &63.3& \multicolumn{1}{c|}{\underline{32.6}} &88.5 & \multicolumn{1}{c|}{\underline{61.5}} & 63.9 & \underline{32.5}\\
AT(\AWPT)   &88.9& \multicolumn{1}{c|}{62.2} &63.9& \multicolumn{1}{c|}{31.9} &87.5 & \multicolumn{1}{c|}{61.3} & 63.3 & \textbf{33.0}\\
AT(\texttt{TrH})    &87.0& \multicolumn{1}{c|}{\underline{61.7}} &62.5& \multicolumn{1}{c|}{\textbf{32.8}} & 88.0& \multicolumn{1}{c|}{\underline{61.0}} & 63.8 & \underline{32.4}\\ \midrule
TRADES(\AWP)  &85.3& \multicolumn{1}{c|}{\underline{60.8}} &63.0& \multicolumn{1}{c|}{\textbf{32.2}} & 84.5& \multicolumn{1}{c|}{59.8} & 61.4 & 32.1\\
TRADES(\AWPT) &85.3& \multicolumn{1}{c|}{60.5} &62.0& \multicolumn{1}{c|}{\textbf{32.2}} & 85.8 & \multicolumn{1}{c|}{61.4} & 65.7 & \underline{33.8} \\
TRADES(\texttt{TrH}) &86.4& \multicolumn{1}{c|}{\underline{61.4}} &62.0& \multicolumn{1}{c|}{\underline{32.1}} &87.4 & \multicolumn{1}{c|}{\textbf{61.7}} & 66.4 & \textbf{34.1} \\ \bottomrule
\end{tabular}

\centering
\begin{tabular}{lcccc|cccc}
\\
\toprule
\toprule
ImageNet  & \multicolumn{4}{c|}{ViT-B16}                            & \multicolumn{4}{c}{ViT-L16}       \\ 
 \footnotesize{SE}$=\se{0.2}$\% &
  \multicolumn{2}{c}{$\ell_\infty (\delta=4/255)$} &
  \multicolumn{2}{c|}{$\ell_2 (\delta=3.0)$} &
  \multicolumn{2}{c}{$\ell_\infty (\delta=4/255)$} &
  \multicolumn{2}{c}{$\ell_2 (\delta=3.0) $} \\ 
Defense &
  \texttt{Clean}(\%) &
  \texttt{AA}(\%) &
  \texttt{Clean} (\%)&
  \multicolumn{1}{c|}{\texttt{AA}(\%)} &
  \texttt{Clean}(\%) &
  \texttt{AA}(\%) &
  \texttt{Clean} (\%)&
  \texttt{AA}(\%) \\ \midrule
AT(\AWP)      &  71.3& \multicolumn{1}{c|}{39.5} & 70.5 & \multicolumn{1}{c|}{39.3} & 74.5& \multicolumn{1}{c|}{44.0} &73.8  & 44.0 \\
AT(\AWPT)     & 71.6 & \multicolumn{1}{c|}{40.6} & 71.0 & \multicolumn{1}{c|}{40.0} & 75.2 & \multicolumn{1}{c|}{44.5} &74.1  & 44.2 \\
AT(\texttt{TrH})      &  71.3& \multicolumn{1}{c|}{\textbf{42.2}} & 71.6 & \multicolumn{1}{c|}{\textbf{42.4}} & 75.8 & \multicolumn{1}{c|}{\textbf{48.8}} & 74.2& \textbf{46.7} \\ \midrule
TRADES(\AWP)  & 65.8 & \multicolumn{1}{c|}{38.6} & 64.5 & \multicolumn{1}{c|}{38.3} &  68.5& \multicolumn{1}{c|}{43.2} & 67.2 &  42.7\\
TRADES(\AWPT) & 68.0 & \multicolumn{1}{c|}{39.8} &67.0  & \multicolumn{1}{c|}{39.7} & 70.5 & \multicolumn{1}{c|}{44.9} & 68.9 & 44.9 \\
TRADES(\texttt{TrH}) &  65.3& \multicolumn{1}{c|}{\textbf{41.9}} & 66.4 & \multicolumn{1}{c|}{\textbf{41.6}} & 70.1  & \multicolumn{1}{c|}{\textbf{48.9}} & 68.9  &  \textbf{47.3}\\ \bottomrule
\end{tabular}

\caption{\texttt{Clean}: \% of Top-1 correct predictions. \texttt{AA}: \% of Top-1 correct predictions under AutoAttack. A max Standard Error (SE)~\cite{stark2005sticigui} = $\sqrt{0.5*(1-0.5)/m}$ (i.e. $m$ as the number of test images) is computed for each dataset. Other results falling into the best $\pm$ SE are not regarded as significantly worse than the best. Best results are highlighted and other candidates within its ballpark (i.e. differences smaller than 2*SE) are underlined to indicate these results may be equally good.}
\label{tab:awpt_results}

\end{table*}

==> Tables/table_cifar10.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{lcccc|cccc}
\toprule
\toprule
\multirow{2}{*}{}  & \multicolumn{4}{c|}{Wide ResNet}                            & \multicolumn{4}{c}{ViT-L16}       \\ 
 &
  \multicolumn{2}{c}{CIFAR-10} &
  \multicolumn{2}{c|}{CIFAR-100} &
  \multicolumn{2}{c}{CIFAR-10} &
  \multicolumn{2}{c}{CIFAR-100} \\ 
Defense &
  $\texttt{Acc}$(\%) &
  \texttt{AA}(\%) &
  $\texttt{Acc}$ (\%)&
  \multicolumn{1}{c|}{\texttt{AA}(\%)} &
  $\texttt{Acc}$(\%) &
  \texttt{AA}(\%) &
  $\texttt{Acc}$ (\%)&
  \texttt{AA}(\%) \\ \midrule
AT(\base)     && \multicolumn{1}{c|}{} && \multicolumn{1}{c|}{} & 87.4 & \multicolumn{1}{c|}{60.8} & 64.3 & 31.7\\
AT(\WA)       && \multicolumn{1}{c|}{} && \multicolumn{1}{c|}{} & 88.0 & \multicolumn{1}{c|}{61.7} & 62.5 & 31.7 \\
AT(\AWP)      && \multicolumn{1}{c|}{} && \multicolumn{1}{c|}{}& 88.5 & \multicolumn{1}{c|}{62.4} & 63.3 & 32.6 \\
AT(\AWPT)    && \multicolumn{1}{c|}{} && \multicolumn{1}{c|}{} & 88.9 & \multicolumn{1}{c|}{62.2} & 63.9 & 31.9 \\
AT(\texttt{TrH})      && \multicolumn{1}{c|}{} && \multicolumn{1}{c|}{} & 87.0 & \multicolumn{1}{c|}{61.7} & 62.5 &  32.8\\ \midrule
TRADES(\base) && \multicolumn{1}{c|}{} & & \multicolumn{1}{c|}{} & 85.2 & \multicolumn{1}{c|}{60.3} & 62.0 &  31.4\\
TRADES(\WA)   && \multicolumn{1}{c|}{} && \multicolumn{1}{c|}{} & 85.9 & \multicolumn{1}{c|}{60.7} & 61.5 &32.0  \\
TRADES(\AWP)  && \multicolumn{1}{c|}{} && \multicolumn{1}{c|}{}& 85.3 & \multicolumn{1}{c|}{60.8} & 63.0 & 32.2 \\
TRADES(\AWPT) && \multicolumn{1}{c|}{} && \multicolumn{1}{c|}{}& 85.3 & \multicolumn{1}{c|}{60.5} & 62.0 & 32.2 \\
TRADES(\texttt{TrH}) && \multicolumn{1}{c|}{} && \multicolumn{1}{c|}{} & 86.4 & \multicolumn{1}{c|}{61.4} & 62.0 & 32.1 \\ \bottomrule
\end{tabular}
\caption{TODO}
\label{fig:main-result-cifar10}
\end{table}
